Topics in Compressed Sensing

Compressed sensing has a wide range of applications that include error correction, imaging, radar and many more. Given a sparse signal in a high dimensional space, one wishes to reconstruct that signal accurately and efficiently from a number of linear measurements much less than its actual dimension. Although in theory it is clear that this is possible, the difficulty lies in the construction of algorithms that perform the recovery efficiently, as well as determining which kind of linear measurements allow for the reconstruction. There have been two distinct major approaches to sparse recovery that each present different benefits and shortcomings. The first, L1-minimization methods such as Basis Pursuit, use a linear optimization problem to recover the signal. This method provides strong guarantees and stability, but relies on Linear Programming, whose methods do not yet have strong polynomially bounded runtimes. The second approach uses greedy methods that compute the support of the signal iteratively. These methods are usually much faster than Basis Pursuit, but until recently had not been able to provide the same guarantees. This gap between the two approaches was bridged when we developed and analyzed the greedy algorithm Regularized Orthogonal Matching Pursuit (ROMP). ROMP provides similar guarantees to Basis Pursuit as well as the speed of a greedy algorithm. Our more recent algorithm Compressive Sampling Matching Pursuit (CoSaMP) improves upon these guarantees, and is optimal in every important aspect.

==> Sudocode.tex <==
SUDOCODE HERE

==> ith.tex <==
%These results are comparable with CoSaMP!
 An alternative greedy approach to compressed sensing uses thresholding methods. There has been much work on various thresholding algorithms, for example see~\cite{FR07:Iterative,DDM04:Iterative-Thresholding}. One of the most recent works on the Iterative Hard Thresholding algorithm (IHT), is an analysis by Blumensath and Davies~\cite{BD08:Iterative}. 
    	
    	\subsubsection[Description]{Description}
    		\label{sec:Approaches:Greedy:Iterative:Description}
    		
    		\subsubsection[Main Theorems and Results]{Main Theorems and Results}
    		\label{sec:Approaches:Greedy:Iterative:Main}
    		
    		\subsubsection[Summary]{Summary}
    		\label{sec:Approaches:Greedy:Iterative:Summary}
